Mangosteen: An Open Thai Corpus for Language Model Pretraining

Pre-training data shapes a language model's quality, but raw web text is noisy and demands careful cleaning. Existing large-scale corpora rely on English-centric or language-agnostic pipelines whose heuristics do not capture Thai script or cultural nuances, leaving risky material such as gambling content untreated. Prior Thai-specific efforts customize pipelines or build new ones, yet seldom release their data or document design choices, hindering reproducibility and raising the question of how to construct a transparent, high-quality Thai corpus. We introduce Mangosteen: a 47 billion-token Thai corpus built through a Thai-adapted Dolma pipeline that includes custom rule-based language ID, revised C4/Gopher quality filters, and Thai-trained content filters, plus curated non-web sources such as Wikipedia, Royal Gazette texts, OCR-extracted books, and CC-licensed YouTube subtitles. Systematic ablations using GPT-2 show the pipeline trims CommonCrawl from 202M to 25M documents while raising SEA-HELM NLG from 3 to 11; an 8B-parameter SEA-LION model continually pre-trained on Mangosteen then surpasses SEA-LION-v3 and Llama-3.1 by about four points on Thai benchmarks. We release the full pipeline code, cleaning manifests, corpus snapshot, and all checkpoints, providing a fully reproducible foundation for future Thai and regional LLM research.

==> introduction-before.tex <==
% Pretraining dataset ถือเป็นหนึ่งในหัวใจของการพัฒนา LLM และโมเดลต่าง ๆ ในปัจจุบัน
Pretraining datasets are an important part of training a language model.
% ไม่แน่ใจอันนี้ถูกไหม
The number of samples can significantly increase the performance of a language model, e.g., \citet{wenzek-etal-2020-ccnet} demonstrates that formulating \emph{large-scale of data} and \emph{diversity of data} is an important key to formulating a robust language model.
%
The experimental results from Dolma~\cite{soldaini-etal-2024-dolma} demonstrate that the language model trained with Dolma's data performs similarly to an open-weight model, Llama2. 
%
Moreover, the pre-training data of Dolma is also publicly available, where the data can be used in both academic and industry.
%
This emphasizes the importance of open science and open source in the NLP community, especially for the development of large language models.
% โปรเจค open source llm
Most current open-source LLMs do not release a training corpus or provide detailed information, do not release training scripts, and are incompatible with the Open Source AI Definition by The Open Source Initiative. Moreover, most current LLMs are English-centric, such as Llama, Mistral, and others, or multilingual language support, such as Qwen, Llama, Gemma, and others, but they have language proportions proportional that can have an effect on the performance of low-resource languages to the pretraining model~\cite{li2024languagerankermetricquantifying} and bias toward high-resource languages such as English~\cite{blasi-etal-2022-systematic}.


% pipeline data 
Most large-scale English pretraining datasets, such as CC-100, C4, RefinedWeb, and Dolma, are derived from the Common Crawl corpus. This data is heavily cleaned and filtered to ensure high quality for model pretraining.
%
Typically, data cleaning pipelines for web pages consist of several stages: language identification to select specific languages, document deduplication to remove duplicates, quality filtering to discard low-quality pages, and content filtering to exclude material from domains unsuitable for training a language model.
%
However, these data cleaning pipelines for web pages are designed for English-centric text. 
%
For multilingual datasets that support Thai, such as CC-100, Fineweb2, and HPLT v2, the data cleaning pipelines are usually language-agnostic. These pipelines are designed to construct a collection of multiple monolingual datasets, rather than being optimized for any single, specific language.

For specific language datasets, SEACrowd Catalogue~\cite{lovenia-etal-2024-seacrowd} collected all datasets for Southeast Asian Languages.
CENDO~\cite{cahyawijaya-etal-2024-cendol} collected a massive scale of pre-training data for Indonesian, resulting in the training of robust T5 and Llama2. %
%
% รวมกับ 2 - 3 ได้
% Recently, 
% there have been attempts to collect pre-training data for low-resource languages, like Thai or Indonesian.
% %
For the Thai language, language models, such as Typhoon-2~\cite{pipatanakul2024typhoon2familyopen}, OpenThaiGPT~\cite{yuenyong2025openthaigpt15thaicentricopen}, and OpenThaiLLM-Prebuilt-7B, conduct continued pre-training on existing multilingual language models, but they do not release their pre-training text corpora, and they do not explain their pipeline or provide enough information for reimplementation and research.
% %
% Typhoon-2~\cite{pipatanakul2024typhoon2familyopen} demonstrated the possibility of creating pre-training data for Thai, where they collect XXX samples from Common Crawl. %
% %
% OpenThaiGPT~\cite{yuenyong2025openthaigpt15thaicentricopen} also collected XXX samples from XXX. 
%
 We observe that the limitations of the current pre-training data for Thai are as follows:
\begin{itemize}
    \item \textbf{Size}. The number of data points is the first thing to consider when we formulate pre-training data. We need as much data as possible. 
    \item \textbf{Diversity}. As demonstrated in Dolma, the important key to getting a successful language model is diversity, where the source of training data should come from different sources and domains. However, the current Thai pre-training data comes from the same source, which is Common Crawl.
    \item \textbf{License}. To develop Thai LLM, the license of the data is also important since most of the Thai data's license is NC (not for industry). The license of Thai pre-training data should be available for both industry and academia. 
\end{itemize}

% รวมกับ 3 ไปได้
To develop a large-scale pre-training dataset for Thai, where the license is available for every use case, we present 47.4B tokens for Thai called WangVisa.
%
We collect data from three sources, such as Common Crawl, Fineweb2, and Non-Common Crawl dataset.
%
We have two groups of training data, where the non-common crawl subset contains 1.5B tokens and the web subset contains 45.9B tokens. % , the medium quality is containing XXX tokens, 
% high-quality / low quality
% [TALK ABOUT DATA CLEANING PIPELINE]
We employed the Dolma pipeline to curate a web-subset dataset through a systematic cleaning process because the Dolma pipeline is easy to customize and supports parallel processing. For language identification, we developed a rule-based script to accurately detect Thai content. The quality filter was adapted by modifying the C4 and Gopher filtering rules to address linguistic and structural nuances specific to Thai. Additionally, we implemented a content filter composed of two custom components: an obscene content filter and a gambling-related content filter, both of which were trained on Thai-specific data to effectively remove undesirable content.

% for cleaning the web subset; Language identifier: we use rule-base script for identifing Thai language, Quality Filter: we adjust C4 rule and Gopher rules to working with Thai language, and content filter: we train both our obscene filter and gambling filparameterter to filter webpage content.

% Test
We are testing every step in our pipeline by training the language model to inspect the step pipeline effect and find the best rule/setting to get the best pipeline setting for the Thai language. We are pretraining GPT-2 124M parameters in 10B tokens in every step and testing with benchmarks such as SEACrowd and SEA-HELM.
%
In addition, to confirm the robustness of our data, we also propose a new Thai large language model using a Southeast Asian language model, namely SEA-LION~\cite{aisingapore-sealion-3-1}, with our pre-training data.
%
SEA-LION is an open-source LLM that we select for the reproducibility of the NLP community.
%
The license of our dataset is the Open Data Commons License Attribution family (odc-by), where the license of the trained model is the Llama 3 license.

We experiment with the trained model using SEACrowd and SEA-HELM. 
% Thai LLM Leaderboard~\footnote{\url{https://huggingface.co/spaces/ThaiLLM-Leaderboard/leaderboard}}.
%  Thai LLM Leaderboard~\footnote{\url{https://huggingface.co/spaces/ThaiLLM-Leaderboard/leaderboard}}.
The experimental results demonstrate that our CPT model outperforms the base model.
%
We also found that with our CPT, it wins the base model.

We summarize the contribution of our paper as follows:
\begin{itemize}
    \item XXX
    \item XXX
    \item XXXX
\end{itemize}


==> limitations.tex <==
% We have observed that the existing Thai benchmark has limitations. However, we believe it is sufficient for testing language models, regardless of their size. In the case of smaller language models, natural language understanding (NLU) cannot be effectively utilized for benchmarking.

% Resource Limitation: we have resource limitation to study pipelines. We study base on GPT-2 model in Decoder only. We can not study Encoder and[TODO]
